Weakly Supervised Detection of Baby Cry

Detection of baby cries is an important part of baby monitoring and health care. Almost all existing methods use supervised SVM, CNN, or their varieties. In this work, we propose to use weakly supervised anomaly detection to detect a baby cry. In this weak supervision, we only need weak annotation if there is a cry in an audio file. We design a data mining technique using the pre-trained VGGish feature extractor and an anomaly detection network on long untrimmed audio files. The obtained datasets are used to train a simple CNN feature network for cry/non-cry classification. This CNN is then used as a feature extractor in an anomaly detection framework to achieve better cry detection performance.

==> backup.tex <==
The basic cross-entropy loss function is most commonly used. For the action recognition of fights, it becomes the binary cross entropy function, 
\begin{equation}
    L_{BCE}( = 1/N {\sum_{i=1}^N y_ilog(p(y_i) + (1-y_i) log(1-p(y_i))}
\label{eq1}
\end{equation}
where $y$ is the label and $p(y)$ is the predicted probability of y for all N points.

